Detecting Benchmark Contamination Through Watermarking

Benchmark contamination poses a significant challenge to the reliability of Large Language Models (LLMs) evaluations, as it is difficult to assert whether a model has been trained on a test set. We introduce a solution to this problem by watermarking benchmarks before their release. The embedding involves reformulating the original questions with a watermarked LLM, in a way that does not alter the benchmark utility. During evaluation, we can detect ``radioactivity'', \ie traces that the text watermarks leave in the model during training, using a theoretically grounded statistical test. We test our method by pre-training 1B models from scratch on 10B tokens with controlled benchmark contamination, and validate its effectiveness in detecting contamination on ARC-Easy, ARC-Challenge, and MMLU. Results show similar benchmark utility post-watermarking and successful contamination detection when models are contaminated enough to enhance performance, \eg $p$-val $=10^{-3}$ for +5$\%$ on ARC-Easy.

==> sections/7-weighted-token-inference.tex <==
Assume we have sequence $t=t_1,\dots,t_n$ sampled from auto-regressive  model $f$. We use $t\sim f[n]$ to denote that $t$ is sampled from decoding $f$ for n tokens. 



Now consider a guesser $g$, that given a sequence $t_{<i}$ and some auxiliary information $aux$, outputs a token $t'_i$. We define

$$\bar{g}(t_1,\dots, t_n, aux) = t'_1,\dots, t'_n \text{~~~where~~~} t'_i = g(t_1,\dots, t_{i-1}, aux)$$

$$p_f( t_{<i}, t_i) = Pr[f(t_{<i}) = t_i ]$$

And we define the score for a guesser $g$ with auxiliary information $aux$ as follows.
$$score_f(g, t, aux, i) = \E_{t'\sim \bar{g}(t, aux)}
[\frac{1}{p_f( t_{<i}, t_i)}\cdot I(t'_i = t_i) ].$$

And 
$$score_f(g, t, aux) = \sum_{i=1}^n score_f(g, t, aux,i)$$


\begin{proposition}
For any fixed auxiliary information $aux$, we have
$$\E_{t \sim f[n]}[score_f(g, t, aux, i)] = 1.$$
\end{proposition}
\begin{proof}
    We have
    \begin{align*}
        \E_{t \sim f[n]}[score_f(g, t, aux, i)] &= \E_{t \sim f[n]}\Big[\E_{t'\sim \bar{g}(t, aux)}
[\frac{1}{p_f( t_{<i}, t_i)}\cdot I(t'_i = t_i) ]\Big]\\
&= \E_{t \sim f[n]}\Big[\E_{t'_i\sim g(t_{<i}, aux)}
[\frac{1}{p_f( t_{<i}, t_i)}\cdot I(t'_i = t_i) ]\Big]\\
&= \E_{t<i \sim f[i-1]}\Big[\E_{t_i \sim f(t_{<i})}\Big[\frac{1}{p_f( t_{<i}, t_i)}\E_{t'_i\sim g(t_{<i}, aux)}
[I(t'_i = t_i) ]\Big]\Big]\\
&= \E_{t<i \sim f[i-1]}\Big[\sum_{t_i \in T}\E_{t'_i\sim g(t_{<i}, aux)}
[I(t'_i = t_i) ]\Big]\\
&= \E_{t<i \sim f[i-1]}\Big[\sum_{t_i \in T}\Pr_{t'_i\sim g(t_{<i}, aux)}
[t'_i = t_i]\Big]\\
&= \E_{t<i \sim f[i-1]}\Big[\Pr_{t'_i\sim g(t_{<i}, aux)}
[t'_i \in T]\Big]\\
&= \E_{t<i \sim f[i-1]}\Big[1\Big] = 1.
    \end{align*}
\end{proof}

\begin{proposition}
Assume for any prefix $t_{<i}$ and $t_i$, we have $p_f(t_{<i} , t_i) \geq \tau$. Then For any fixed auxiliary information $aux$, we have
$$  \Pr_{t\sim f[n]}[ score_f(g,t,aux) \geq n(1+\gamma) ] \leq e^{-n\gamma^2\tau^2}$$
\end{proposition}
\begin{proof}
    We use the fact that the score at each step is bounded by $\frac{1}{\tau}$ and apply Azuma inequality. 
\end{proof}
